A Game-Theoretic Analysis of Auditing Differentially Private Algorithms with Epistemically Disparate Herd

Privacy-preserving AI algorithms are widely adopted in various domains, but the lack of transparency might pose accountability issues. While auditing algorithms can address this issue, machine-based audit approaches are often costly and time-consuming. Herd audit, on the other hand, offers an alternative solution by harnessing collective intelligence. Nevertheless, the presence of epistemic disparity among auditors, resulting in varying levels of expertise and access to knowledge, may impact audit performance. An effective herd audit will establish a credible accountability threat for algorithm developers, incentivizing them to uphold their claims. In this study, our objective is to develop a systematic framework that examines the impact of herd audits on algorithm developers using the Stackelberg game approach. The optimal strategy for auditors emphasizes the importance of easy access to relevant information, as it increases the auditors' confidence in the audit process. Similarly, the optimal choice for developers suggests that herd audit is viable when auditors face lower costs in acquiring knowledge. By enhancing transparency and accountability, herd audit contributes to the responsible development of privacy-preserving algorithms.

==> bibnote.tex <==
@article{RI_review,
Author = {Maćkowiak, Bartosz and Matějka, Filip and Wiederholt, Mirko},
Title = {Rational Inattention: A Review},
Journal = {Journal of Economic Literature},
Volume = {61},
Number = {1},
Year = {2023},
Month = {March},
Pages = {226-73},
DOI = {10.1257/jel.20211524},
URL = {https://www.aeaweb.org/articles?id=10.1257/jel.20211524}}

@article{Sims_2003,
  title={Implications of rational inattention},
  author={Sims, Christopher A},
  journal={Journal of monetary Economics},
  volume={50},
  number={3},
  pages={665--690},
  year={2003},
  publisher={Elsevier}
}

@article{RI_discrete,
  title={Rational inattention to discrete choices: A new foundation for the multinomial logit model},
  author={Mat{\v{e}}jka, Filip and McKay, Alisdair},
  journal={American Economic Review},
  volume={105},
  number={1},
  pages={272--298},
  year={2015},
  publisher={American Economic Association 2014 Broadway, Suite 305, Nashville, TN 37203}
}


@incollection{eps_science,
  title={Epistemic injustice in science},
  author={Grasswick, Heidi},
  booktitle={The Routledge handbook of epistemic injustice},
  pages={313--323},
  year={2017},
  publisher={Routledge}
}

